DPD-fVAE: Synthetic Data Generation Using Federated Variational Autoencoders With Differentially-Private Decoder

Federated learning (FL) is getting increased attention for processing sensitive, distributed datasets common to domains such as healthcare. Instead of directly training classification models on these datasets, recent works have considered training data generators capable of synthesising a new dataset which is not protected by any privacy restrictions. Thus, the synthetic data can be made available to anyone, which enables further evaluation of machine learning architectures and research questions off-site. As an additional layer of privacy-preservation, differential privacy can be introduced into the training process. We propose DPD-fVAE, a federated Variational Autoencoder with Differentially-Private Decoder, to synthesise a new, labelled dataset for subsequent machine learning tasks. By synchronising only the decoder component with FL, we can reduce the privacy cost per epoch and thus enable better data generators. In our evaluation on MNIST, Fashion-MNIST and CelebA, we show the benefits of DPD-fVAE and report competitive performance to related work in terms of Fr\'echet Inception Distance and accuracy of classifiers trained on the synthesised dataset.

==> sections/3_methods/dp_algorithm.tex <==
Preconditions:
\begin{itemize}
	\item Dataset specification ($N$, input dimension, output dimension)
	\item Model specification with corresponding number of trainable parameters: $|\theta|$
	\item DP budget $\epsilon$
	\item DP risk $\delta$
\end{itemize}

\begin{enumerate}
	\item By training the model with either added Gaussian noise or $L2$-norm clipping, find $L2$-norm bounds for added noise $S_\sigma$ and $S_\theta$.
	\item Fix an initial search space for: 
		\begin{itemize}
			\item norm clip $S$ (e.g. $[0.01, 5.0]$)
			\item noise multiplier $z$ (e.g. $[0.1, 2.0]$)
			\item client sampling frequencies $q$ (e.g. $[0.001, 0.25]$)
		\end{itemize}
	\item Find combinations of $q$ and $z$ that keep budget $\epsilon$:
		\begin{itemize}
			\item For fairness, and to include every clients' data, set the minimum number of epochs so that we expect every client to be sampled at least once, so $E = 1/q$
			\item Calculate privacy spending $\epsilon_E$ in epoch $E$ from RDP-Accountant with $(q, z, \delta)$
			\item If $\epsilon_E < \epsilon$, add $(q, z)$ to valid combinations
		\end{itemize}
	\item Find upper bound on noise std.dev $\sigma$ by determining the $L2$-norm of $|\theta|$ random sampled drawn from $\mathcal{N}(0, \sigma)$
	\item Find largest $S$ that keeps $\frac{zS}{Nq} < \sigma$ for any $(q, z)$ combination.
\end{enumerate}
